MCMC assisted by Belief Propagation

Markov Chain Monte Carlo (MCMC) and Belief Propagation (BP) are the most popular algorithms for computational inference in Graphical Models (GM). In principle, MCMC is an exact probabilistic method which, however, often suffers from exponentially slow mixing. In contrast, BP is a deterministic method, which is typically fast, empirically very successful, however in general lacking control of accuracy over loopy graphs. In this paper, we introduce MCMC algorithms correcting the approximation error of BP, i.e., we provide a way to compensate for BP errors via a consecutive BP-aware MCMC. Our framework is based on the Loop Calculus (LC) approach which allows expressing the BP error as a sum of weighted generalized loops. Although the full series is computationally intractable, it is known that a truncated series, summing up all 2-regular loops, is computable in polynomial-time for planar pair-wise binary GMs and it also provides a highly accurate approximation empirically. Motivated by this, we first propose a polynomial-time approximation MCMC scheme for the truncated series of general (non-planar) pair-wise binary models. Our main idea here is to use the Worm algorithm, known to provide fast mixing in other (related) problems, and then design an appropriate rejection scheme to sample 2-regular loops. Furthermore, we also design an efficient rejection-free MCMC scheme for approximating the full series. The main novelty underlying our design is in utilizing the concept of cycle basis, which provides an efficient decomposition of the generalized loops. In essence, the proposed MCMC schemes run on transformed GM built upon the non-trivial BP solution, and our experiments show that this synthesis of BP and MCMC outperforms both direct MCMC and bare BP schemes.

==> main_2regular_sec1_old.tex <==
\section{Estimating the 2-regular Partition Function}\label{sec:2regular}

The aim of this Section is to present an efficient approximation algorithm to compute
$2$-regular loop series in binary GM where each vertex is at most of degree $3$. This may seems restrictive,  but in fact any pairwise GM (with vertexes of an arbitrary, finite degree) can be reduced to a binary GM with vertexes of degree at most $3$. The reduction can be achieved through the following algorithm:
\begin{itemize}
\item[1.] Pick a vertex $s$ with degree larger than 3, expand the vertex into $s_{1}, s_{2}, \cdots s_{d_{v}(G)}$.
\item[2.] For each $i = 1,2,\cdots d_{v}(G)$:
\begin{itemize}
\item[i)] Delete the edge $(s,t_{i})$
\item[ii)] Add a new edge $(s_{i}, t_{i})$. Assign to the newly added edge potential of the previously deleted edge, $\psi_{s,t_{i}}$.
\end{itemize}
\item[3.] Add the edges $(s_{1},s_{2}), (s_{2},s_{3}),\cdots (s_{d_{v}(G)}, s_{1})$ 
with potentials 
\begin{align*}
    \delta(x,x^\prime) = 
    \begin{cases}
    1\qquad \mbox{if}~x=x^\prime\\
    \mbox{otherwise}
    \end{cases}
\end{align*}
\end{itemize}
\begin{figure}[h]
    \centering
    \includegraphics{make3regular}
    \caption{Example of expanding a vertex.}
    \label{fig:make3regular}
\end{figure}
It is straightforward to check that partition function of the newly built GM (with reduced degree) is equal to the partition function of the original GM. 
One benefit of working with the graph of the maximum degree $3$ is that in this case the number of $2$-regular generalized loops, also corresponding to the 
Eulerian sub-graphs, can be counted  explicitly. It is $2^{m-n+c}$ where $m,n$ and $c$ denotes the number of edges, vertexes and connected components of the graph. 
Detailed description of the procedure will be discussed in Section \ref{sec:cyclebasis}.


The rest of section consist of two parts. 
We first propose a sampler for 
$2$-generalized loops with probability proportional to its absolute value of its weights, i.e.
\begin{align}\label{eq:2regularMCdistribution}
\pi(F) = \frac{|w(F)|}{Z^{\dagger}_\emptyset}
\end{align}
based on Jerrum and Sinclair's MC \cite{C3}.
Then we give a scheme for estimating the logarithm of
$2$-regular partition function $Z_\emptyset = \sum_{F\in \mathcal{L}}w(F)$ based on the proposed sampler.
\iffalse
Note that $2$-regular partition function may consist of both positive and negative terms, 
so its direct approximation is non-trivial. 
To overcome this issue, we first approximate the sum of absolute value of each terms,
$Z^{\dagger}_{\emptyset} = \sum_{F \in \mathcal{L}}|w(F)|$. 
Then the ratio $Z_{\emptyset}/Z^{\dagger}_{\emptyset}$ is approximated 
via estimating positive and negative parts of the $2$-regular loop series. 
Each approximation is based on the 
which is a modification of Jerrum and Sinclair's MC \cite{xx}.
\fi

\subsection{2-regular generalized loop sampler}
%We now give detailed explanation of the proposed sampler. 
The proposed sampling algorithm is based on 
the Markov chain proposed by Jerrum and Sinclair \cite{C3}, 
spanning the power set of edges $2^{E}$ in the graph. 
In our application, 
we modify the Markov chain so that the probability of 
sampling a $2$-generalized loop is sufficiently large. 
Then the sampler for $2$-regular generalized loop 
with distribution \eqref{eq:2regularMCdistribution} 
is obtained by iterating the following trial: simulate the chain for 
sufficient amount of steps and output the final state 
if it is a $2$-generalized loop.

The Markov chain $\mathcal{MC}$ has the following distribution:
\begin{align}\label{eq:subgraphMCdistribution}
\pi^\dagger(F) = \frac{1}{Z_{\emptyset}^\dagger}\lambda^{|\mbox{odd}(F)|}|\hat{w}(F)|
\end{align}
where $\mbox{odd}(F)$ is the set of vertices 
having odd degree in the edge-induced graph of $F$,
$\lambda$ is some constant which will be defined later, and 
\begin{align}
\hat{w}(F) = \prod_{st\in F}\frac{\tau_{st}-\tau_{s}\tau_{t}}{\left(\tau_{s}\tau_{t}(1-\tau_{s})(1-\tau_{t})\right)^{1/2}}.
\end{align}
Note that $\hat{w}(F) = w(F)$ 
if $F$ is a $2$-regular generalized loop and
the samples of $2$-generalized loops will have the 
desired distribution.

For $F, F^\prime \in \Omega$ with $F\neq F^\prime$, 
the transition probability from $F$ to $F^\prime$ is given by
\begin{align}\label{eq:2regulartransition}
p(F,F^\prime) = 
\begin{cases}
1/2m \qquad &\mbox{if $|F\oplus F^\prime| = 1$ and $\hat{w}(F^\prime) \geq \hat{w}(F)$}\\
|\hat{w}(F^\prime)|/2m|\hat{w}(F)|\qquad &\mbox{if $|F\oplus F^\prime| = 1$ and $\hat{w}(F^\prime) < \hat{w}(F)$}\\
0 \qquad &\mbox{otherwise}
\end{cases}
\end{align}
where the self-loop probabilities $p(X,X)$ are defined implicitly by complementation, 
so that $p(X, X) = 1 - \sum_{X^\prime \neq X}p(X, X^\prime)$. 
Here, transitions in the markov chain 
are either adding or deleting a single edge 
from the set $X$. 
%Thus, transitions in the markov chain are perturbation in which a single edge is added to, 
%or deleted from a subgraph. 
One can observe that this markov chain is ergodic, 
i.e. it spans over all state space and 
converges to the stationary distribution. 
Jerrum and Sinclair \cite{C3} 
proved the bound on mixing time.
\begin{theorem}[Jerrum, Sinclair 1990]
The mixing time $\tau_{x}(\delta)$ is bounded above by 
\begin{align}
\tau_{X_{0}}(\delta) \leq \frac{(\log (\delta) + \log(\pi^\dagger(X_{0}))}{4\lambda^{4}m}.
\end{align}
\end{theorem}

Additionally, if we set $\lambda$ appropriately, 
the probability of sampling a 
$2$-regular generalized loops is sufficiently large. 
\begin{theorem}\label{thm:sample2regular}
Let $d$, $w_{\min}$ denote the diameter of the graph $G$ and 
minimum weight among the edges respectively. 
Once we set $\lambda = \frac{w_{\min}^{d}}{n}$, the probability of sampling an even degree subgraph is at least 
$\frac{2}{n+2}$. In other words, 
\begin{align}
\frac{Z_{\emptyset}}{Z^{\dagger}_{\emptyset}}\geq\frac{2}{n+2} 
\end{align}
Here, $d$ is the diameter of the graph, i.e. the maximum 
distance between any two vertices in the graph.
\end{theorem}
As a result, we obtain the following algorithm for 
sampling from the 
distribution in \eqref{eq:2regularMCdistribution} 
with tolerance $\delta$. 

\begin{algorithm}[tbh]
\caption{Sampling $2$-regular generalized loops}
\label{alg:sample2regular}
\begin{algorithmic}[1]
\STATE {\bf Input:} Desired distribution $\pi$ and tolerance $\delta$ of the samples
\STATE {\bf Output:} A sample from the distribution $\pi$ with tolerance $\delta$.
\STATE {\bf Initialize:} Set $\lambda \leftarrow \frac{w_{\min}^{d}}{n}$, $\hat{\delta} \leftarrow 2\delta / 3(n+2)$.
\FOR{$i = 1 \to \lceil(n/2 + 1)\ln(3/\delta)\rceil$} %\Comment{123}
\STATE Choose a $2$-regular generalized loop $X_{0}$ and set $X\leftarrow X_{0}$. 
\FOR{$t = 1 \to \lceil\frac{(\log (\delta) + \log(\pi^\dagger(X_{0}))}{4\lambda^{4}m}\rceil$}
\STATE Update $X$ by the transition matrix \eqref{eq:2regulartransition} with parameter $\lambda$.
\ENDFOR
\IF{$X$ is a generalized loop} 
\STATE BREAK and output $X$.
\ENDIF
\ENDFOR
\STATE Output a random $2$-regular generalized loop.
\end{algorithmic}
\end{algorithm}

\iffalse
\noindent{\bf 2-regular generalized loop sampler}
%\vspace{5pt}
\hrule
\begin{itemize}
\item[1.] Set $\lambda \leftarrow \frac{w_{\min}^{d}}{n}$, $\hat{\delta} \leftarrow 2\delta / 3(n+2)$.
\item[2.] Repeat $T = \lceil(n/2 + 1)\ln(3/\delta)\rceil$ times:
\begin{itemize}
\item[(i)] Simulate the Markov chain $\mathcal{MC}$, with parameter $\lambda$, 
for 
$\frac{(\log (\delta) + \log(\pi^\dagger(X_{0}))}{4\lambda^{4}m}$ steps (with initial state $X_{0}$).
\item[(ii)] Output the final state if it is a $2$-regular generalized loop and halt.
\end{itemize}
\item[3.] Output an arbitrary $2$-regular generalized loop if all trials fail.
\end{itemize}
\hrule
\vspace{0.1in}
\fi

\begin{corollary}\label{cor:sample2regular}
The algorithm {\bf 2-regular generalized loop sampler} outputs the sample from the distribution $\pi$ 
with tolerance $\delta$.
\end{corollary}
%Having the results,%Corollary \ref{cor:sample2regular}, 
In addition, Jerrum and Sinclair \cite{C3} quantified how much samples are necessary for 
estimating some non-negative real valued function $f$ 
using the proposed sampler. 
The theorem is directly applicable to our case, 
using the {\bf 2-regular generalized loop sampler} 
to achieve a specified accuracy with specified confidence.
\begin{theorem}[Jerrum, Sinclair 1990]
\label{thm:samplenum2regular}
Let $f$ be a non-negative real-valued random variable defined on the set 
$\Omega$ and let $\xi$, $\eta$ be real numbers with 
$0<\xi\leq 1$ and $0<\eta \leq 1/2$.
Then using 
$504\xi^{-2}\lceil\log \eta^{-1}\rceil \max(f)/\mathbb{E}(f)$ samples from 
the {\bf 2-regular generalized loop sampler}, 
%each with input $(w, \lambda)$ and tolerance 
%$\delta = \xi \mathbb{E}(f)/8\max(f)$, and 
produces an ouput $Y$ satisfying 
\begin{align*}
    \mbox{Pr}\left(Y~\mbox{approximates $\mathbb{E}(f)$ within ratio $1+\xi$}\right) \leq 1-\eta.
\end{align*}
\end{theorem}

Theorem \ref{thm:samplenum2regular} implies that whenever we 
use the {\bf 2-regular generalized loop sampler} for approximating 
a non-negative function $f$, the ratio $\max f / \mathbb{E}(f)$ must be 
bounded by a polynomial function of the size of the system.

==> proof_2regular_old.tex <==
\section{Proofs of Theorems}
\iffalse
\subsection{Proof of of Theorem \ref{thm:mixing2regular}}
Our proof makes use of the following result \cite{xx}. 
\begin{theorem}[Schweinsberg 2002 \cite{xx}.] 
Consider an irreducible and lazy Markov chain, 
with finite state space $\Omega$ and transition matrix $P$, 
which is reversible with respect to the distribution $\pi$. 
Let $\mathcal{O} \subseteq \Omega$ be nonempty, and 
for each pair $(I,F) \in \Omega \times \mathcal{O}$, specify a path 
$\gamma_{I,F}$ in $\mathcal{G}_{P}$ form $I$ to $F$. 
Let 
\begin{align}
\Gamma = \{\gamma_{I,F} : (I,F) \in \Omega \times \mathcal{O}\}
\end{align}
denote the collection of all such paths, and let $\mathcal{L}(\Gamma)$ be the longest 
path is $\Gamma$. 
For any transition $T$, let 
\begin{align}
\mathcal{P}_{T} = \{(I,F)\in \Omega \times \mathcal{O}: T \in \gamma_{I,F}\}.
\end{align}
Then 
\begin{align}
\tau_{A}(\delta) \leq \left[\log\left(\frac{1}{\pi(A) + \log \left(\frac{1}{\delta}\right)}\right)\right] 4\mathcal{L}(T)\Phi(\Gamma)
\end{align}
where 
\begin{align}
\Phi(\Gamma) = \max_{(A,A^\prime) \in \mathcal{E}_{P}}
\left\{
\sum_{I,F \in \mathcal{P}_{(A,A^\prime)}} \frac{\pi (I)\pi(F)}{\pi(\mathcal{O})\pi(A)P(A,A^\prime)}.
\right\}
\end{align}
\end{theorem}
In our application, we choose $\mathcal{O} = L_{0}$ and 
we show that there exists a choice of paths $\Gamma = \{\gamma_{I,F}: (I,F) \in L_{0}\cup L_{2} \times L_{0}\}$ such that
\begin{align}
\Phi(\Gamma) \leq dn^{4}, \qquad \mathcal{L}(\Gamma) \leq m.
\end{align}
Then we are able to obtain our main result immediately.

We specify $\Gamma$ first. 
To this end, we fix a ordering of vertices by labeling them $1,\cdots n$.
Now observe that 
for any pair $(I,F) \in L_{0}\cup L_{2} \times L_{0}$,
the symmetric difference $I\oplus F$ is consisting of 
components $C_{0}, C_{1}, \cdots C_{k}$. 
Moreover, there exist at most $1$ path 
among the components (say $C_{0}$), and other components are 
simple cycles. 
This can be shown by the fact that $\mbox{odd}(I\oplus F) = \mbox{odd}(I)$, 
since $F$ is $2$-regular.
We now define $\gamma_{I,F}$ by updating (applying symmetric difference)
the edges in $C_{0}, C_{1},\cdots C_{k}$. 
If $C_{0}$ is a path, pick the endpoint with higher order of label. 
Then the edges in paths are updated by {it unwinding} the path $C_{0}$, 
starting from the chosen endpoint.
In case of cycles, we pick a vertex with highest order of label and 
unwind the edges according to some fixed cycle orientation. 
Note that intermediate states are still in $L_{0} \cup L_{2}$ since we update $C_{0}$ first.

We now bound $\Phi(\gamma)$. 
Define 
\begin{align}
\mathcal{P}_{T,k} = \{(I,F) \in L_{k}\times L_{0}, T \in \gamma_{I,F}\},
\end{align}
then $\mathcal{P}_{T} = \mathcal{P}_{T,0} \cup \mathcal{P,2}.$
We now define a mapping $\eta_{T}: \mathcal{P}_{T}\rightarrow L_{0}, L_{2}, L_{4}$ as:
\begin{align}
\eta_{T}(I,F) = I\oplus F\oplus (A\cup e).
\end{align}
where $T = (A, A\oplus e)$. 
We prove that $\eta_{T}$ is an injection. 
This is shown by reconstructing $I$ and $F$ from $\eta_{T}(I,F)$. 
First observe that $I\oplus F = \eta_{T}(I,F) \oplus (A \cup e)$, 
so all we need is to partition $I\oplus F$ into 
$I\backslash F$ and $F \backslash I$. 
Then from the fixed label of vertices, we are able to 
infer the order in which the edges in $I\oplus F$ must be unwound. 
Thus we obtain $I$ and $F$ as a result. 

Now we prove that for any $T \in \mathcal{E}$, we can bound the term 
\begin{align}
\frac{1}{\pi(L_{0})} \frac{\pi(I)\pi(F)}{\pi(A)P(A,A^\prime)} \leq 
\frac{2d}{\lambda(L_{0})} \Psi(I) \lambda(\eta_{T}(I,F)).
\end{align}
We have 
\begin{align}
\frac{1}{\pi(L_{0})} \frac{\pi(I)\pi(F)}{\pi(A)P(A,A^\prime)} =
\frac{1}{n\lambda(L_{0})} \frac{\Psi(I)\lambda(I)n\lambda(F)}{\Psi(A)\lambda(A)P(A,A^\prime)}\\
\leq \frac{1}{\lambda(L_{0})} \Psi(I)\lambda(I)\lambda(F) \frac{2d}{\lambda(A\cup e)} \\
= \frac{2d}{\lambda(L_{0})}\Psi(I) \lambda(\eta_{T}(I,F))
\end{align}
and the statement is proven. 
Now observe that 
\begin{align}
\Psi(\Gamma) \leq \sum_{(I,F)\in \mathcal{P}_{T}} 
\frac{2d}{\lambda(L_{0})}
\end{align}
\fi


\subsection{Proof of of Theorem \ref{thm:sample2regular}}
First, observe that for any $W\subset V$, 
\begin{align}
\sum_{F\in L(W)} |\hat{w}(F)| 
&= \frac{1}{2^{n}}\sum_{F\in L(W)} \prod_{e\in F} |\hat{w}(e)| \prod_{s\in V\backslash W} (1 + (-1)^{d_{s}(F)})
\prod_{s\in W}(1 + (-1)^{d_{s}(F)+1})\\
&= \frac{1}{2^{n}}\sum_{\sigma\in\{-1,1\}^n}\sum_{F\in L(W)} \prod_{e\in F} |\hat{w}(e)| 
\prod_{s\in V} \sigma_{s}^{d_{s}(F)} \prod_{s\in W} \sigma_{s} \\
&\leq \sum_{\sigma\in\{-1,1\}^n}\frac{1}{2^{n}}\sum_{F\in L(W)} \prod_{e\in F} |\hat{w}(e)| 
\prod_{s\in V} \sigma_{s}^{d_{s}(F)} \\
&= \sum_{F\in L(\emptyset)}|\hat{w}(F)|.
\end{align}
The inequality comes from the fact that $\sigma \leq 1$. 
Therefore we have $\sum_{F\in L(\emptyset)}|\hat{w}(F)| \geq \sum_{F\in L(W)}|\hat{w}(F)|$ and 
\begin{align}
\frac{\sum_{F \in L_{0}}\pi^{\dagger}(F)}{\sum_{F \in L_{0}\cup L_{2}}\pi^{\dagger}(F)} 
&= \frac{n\sum_{F \in L_{0}}|\hat{w}(F)|}{n\sum_{F \in L_{0}}|\hat{w}(F)| + \sum_{W\subseteq V, |W|=2}\sum_{F \in L_{W}}|\hat{w}(F)|} \\
\geq \frac{n}{n+2\binom{n}{2}}
&= \frac{1}{n}.
\end{align}
Thus the proof is complete.
\iffalse
\subsection{Proof of of Theorem \ref{thm:sample2regular}}
Given $S\subseteq V$, 
let $L(S)$ denote the collection of edges 
such that the degree of vertices in $S$ 
is odd in the corresponding 
edge-induced subgraphs. 
Note that the size of $S$ is even and 
the set of $2$-regular generalized loop is equivalent to
$L(\emptyset)$. 
Our objective would be to prove:
\begin{align}\label{eq:sample2regular}
\sum_{F\in L(\emptyset)}w(F)
\leq
\frac{2}{n+2}\sum_{S: S\subseteq V}\sum_{F\in L(S)}w(F)
\end{align}
First enumerate the vertices in $S^{\prime}\backslash S$ 
and let $P_{i}$ denote the shortest 
path (without weights) having $2i-1$ and $2i$-th vertex as its endpoint.
Then define an 
one-to-one mapping $f$ between $L(S)$ and $L(S^\prime)$:
\begin{align}
f(H) = H \oplus P_{1} \oplus P_{2}\oplus \cdots \oplus P_{|S^{\prime}\backslash S|/2}.
\end{align}
Note that 
$L(\emptyset)$ is the set of $2$-regular generalized loops and
existence of such mapping implies 
\begin{align}
|L(S)|=|L(\emptyset)|=2^{m-n+c}.
\end{align}
Since the symmetric difference of each path 
scales the weight at most $w^{d}_{min}$,
we obtain the following inequality:
\begin{align}
w(F) \geq w_{\min}^{d|S^{\prime}\backslash S|}w(f(F))
\end{align}
Thus, we conclude that 
\begin{align}
\lambda^{k}\sum_{S: |S|=k, S\subseteq V}\sum_{F\in L(S)}w(F)
&\leq \lambda^{k}w^{d}_{\min}\binom{n}{k}\sum_{F\in L(\emptyset)}w(F)\\
&\leq \sum_{F\in L(\emptyset)}w(F)
\end{align}
for any $0<k\leq n$. Thus we obtain the desired inequality in 
\eqref{eq:sample2regular}.
\fi

\subsection{Proof of Corollary \ref{cor:sample2regular}}
Let $S$ be the set of arbitrary $2$-regular generalized loops. 
The result follows from the
chain of inequalities:
\begin{align}
\mbox{Pr}(X \in S) 
&\leq \frac{\hat{\pi}(S)}{\hat{\pi}(\mathcal{L}} - (1-\hat{\pi}(\mathcal{L})^{T}\\
&\leq \frac{\pi(S) - \hat{\delta}}{\pi(\mathcal{L}+\hat{\delta}} - \exp(-\hat{\pi}(\mathcal{L})T)\\
&\leq \frac{\pi(S)}{\pi(\mathcal{L})} - \frac{2\hat{\delta}}{\pi(\mathcal{L})} - \exp(-(\pi(\mathcal{L}) - \hat{delta})T)\\
&\leq \frac{\pi(S)}{\pi(\mathcal{L})} - \frac{2\delta}{3} - \frac{\delta}{3}
\end{align}
The converse follows immediately by considering the complementary set $\mathcal{L} \backslash S$.
\iffalse
\subsection{Proof of Theorem \ref{thm:samplenum2regular}}
Let $\mbox{Var}(f) = \mathbb{E}(f^{2}) - \mathbb{E}(f)^{2}$ 
denote the variance of $f$. The {\bf 2-regular generalized loop sampler} 
selects generalized loop from a distribution $p$. 
Now we define the mean and variance of $f$ with 
respect to $p$:
\begin{align}
\mathbb{E}^\prime(f) &= \sum_{F\in \mathcal{L}}p(F)f(F);\\
\mbox{Var}^\prime(f) &= \sum_{F\in \mathcal{L}}p(F)f(F)^{2} - \mathbb{E}^\prime (f)^{2}.
\end{align}
Since $|| p- \pi || \leq \delta$, we have 
\begin{align}

\end{align}
\fi
\subsection{Proof of Theorem \ref{thm:annealing2regular}}
The result follows from the following set of inequalities.
\begin{align}
\frac{Z^{\dagger}_{\emptyset}(\beta^{\prime})}{Z^{\dagger}_{\emptyset}(\beta)}
&= \frac{\sum_{F \in \mathcal{L}}|w(F)|^{\beta^\prime}}{\sum_{F \in \mathcal{L}}|w(F)|^{\beta^\prime}} \\
&\leq (w_{\min}^{|F_{\max}|})^{\beta^\prime - \beta}\\
&\leq w_{\min}
\end{align}
Here, $F_{\max}$ is the $2$-regular generalized loop with maximum number of edges. 
Since it is $2$-regular, $|F_{\max}|\leq n$.

%\subsection{Proof of Corollary \ref{cor:estimateabspartition}}
\subsection{Proof of Corollary \ref{cor:estimatepartition2regular}}

Using Theorem \ref{thm:sample2regular}, each $H_{i}$ is estimated 
within ratio of $1 + \xi$ with probability at least $1-\eta$. 
Then $Z^\dagger_\emptyset$ is estimated within ratio of 
\begin{align}
(1+\xi)^{n} = (1 + \frac{\varepsilon}{2n})^{n} \leq 1+\varepsilon
\end{align} 
with probability 
\begin{align}
(1-\eta)^{n} = 1-\nu.
\end{align} 

First assume the case $\kappa > \varepsilon$. 
Then using Theorem \ref{thm:sample2regular}, $\kappa$ is estimated 
within ratio of $1+\xi$ with probability at least 
$1-\eta$. 
Then the result is obtained by the 
following chain of inequalities:
\begin{align}
\log(1-2\kappa + 2\kappa\xi) &\leq 1 + \log \frac{1-2\kappa + 2\kappa\xi}{1-2\kappa}\\
&\leq 1 + \log (e^{cn}-1)e^{\varepsilon}
\end{align}
The converse is similar. 
Now when $\kappa < \xi$, 
$\kappa$ is estimated within ratio of 
$\xi^{\prime} = \frac{\xi^{3/2}}{\kappa^{1/2}}$ with probability at least $1-\eta$. 
Then the result is obtained by the following chain of inequalities:
\begin{align}
\log(1-2\kappa(1+ \xi)) &\leq 1 + 
\log \left(\frac{1-2(1 -\xi^{\prime})\kappa}{1-2\kappa}\right)\\
&\leq 1 +  \log \left(1-(\frac{\xi^{3/2}}{\kappa^{1/2}})\kappa\right) \\
&\leq 1 + \log  \left(1 + \xi\right) = 1 + \log \left(1+e^{\varepsilon}\right)
\end{align}
and if we set $\xi < 1/4$, 
\begin{align}
\log(1-2\kappa - 2\kappa\xi) &\geq 1 + 
\log \left(\frac{1-2(1+\xi^{\prime})\kappa}{1-2\kappa}\right)\\
&\geq 1 + \log \left(\frac{1-2(1+ \frac{\xi^{3/2}}{\kappa^{1/2}})\kappa}{1-2\kappa}\right)\\
&\geq 1 + \log \left(1 - \frac{2\xi^{2}}{1-2\xi} \right)\\
&\geq 1 + \log \left(1 - 4\xi^{2}\right) = 1 + \log \left(1 - 4e^{2\varepsilon}\right).
\end{align}


==> proof_full_old.tex <==
\subsection{Proof of Theorem \ref{thm:cyclebasismapping}}
Given any element $D$ of $2^{\mathcal C}$, let $H$ be the corresponding  
$2$-regular generalized loop.
Pick a set of paths 
$\mathcal P = \{P_{1}, P_{2},\cdots P_{k}\}$ having its endpoints as 
vertices in $S$ by choosing without replacement. 
Then the described mapping $f$ can be obtained by:
\begin{align}
f(D) = H \oplus P_{1} \oplus P_{2}\oplus \cdots \oplus P_{k}
\end{align}
The mapping is one to one trivially and 
a natural out come is that the size of $L(S)$ is exactly $2^{m-n+1}$ independent of $S$.

\subsection{Proof of Theorem \ref{thm:generalizedloopdecomp}}
Given any $F \in L(S)$, observe that 
\begin{align}
F \oplus P_{1} \oplus \cdots \oplus P_{l/2} \in L(\emptyset).
\end{align}
Thus there exist some $C_{1}, C_{2}, \cdots C_{k} \in \mathcal{C}$ 
such that 
\begin{align}
C_{1}\oplus C_{2} \cdots \oplus C_{k} = F \oplus P_{1} \oplus \cdots \oplus P_{l/2}
\end{align}
and the proof is done.
